Blade Envelopes Part II: Multiple Objectives and Inverse Design

Blade envelopes offer a set of data-driven tolerance guidelines for manufactured components based on aerodynamic analysis. In Part I of this two-part paper, a workflow for the formulation of blade envelopes is described and demonstrated. In Part II, this workflow is extended to accommodate multiple objectives. This allows engineers to prescribe manufacturing guidelines that take into account multiple performance criteria. The quality of a manufactured blade can be correlated with features derived from the distribution of primal flow quantities over the surface. We show that these distributions can be accounted for in the blade envelope using vector-valued models derived from discrete surface flow measurements. Our methods result in a set of variables that allows flexible and independent control over multiple flow characteristics and performance metrics, similar in spirit to inverse design methods. The augmentations to the blade envelope workflow presented in this paper are demonstrated on the LS89 turbine blade, focusing on the control of loss, mass flow and the isentropic Mach number distribution. Finally, we demonstrate how blade envelopes can be used to visualize invariant designs by producing a 3D render of the envelope using 3D modelling software.

==> cad.tex <==
\section{PRACTICAL UTILITY AND DISSEMINATION}
Thus far in this two-part paper, we have enumerated the core computational techniques required for generating a blade envelope under multiple constraints. We have articulated its utility in design (both forward and inverse) by identifying and exploiting the inactive subspace. Although all our efforts have focused on the LS89, the concept of a blade envelope extends well beyond any given airfoil, and indeed an isolated 2D cross-section. We envision blade envelopes forming a critical part of the design stage, facilitating discussions on trade-offs and tolerances. 
%Our online companion blog post (\hl{available here: }) features code not only for replicating the results of these two papers, but also provides a step-by-step guide on extensions to other arbitrary geometries – requiring only a database of CFD evaluations and a plug-in geometry generation tool.

Beyond design, a key contribution of our work is a machine learning technique for deciding whether a manufactured blade's tolerance variations are permissible or not. This program can be easily incorporated within an existing coordinate measuring machine protocol and used in manufacturing assembly lines, with the aim of moving away from existing broad spectrum tolerances and opting for a more bespoke, design-centric one, which may offer opportunities for relaxing tolerances---thereby reducing manufacturing costs. Additionally, we see tremendous utility of the blade envelope in health monitoring; a topic we address in detail in a forthcoming paper. When inspecting blades that have gone through several hundred hours of operation, using either detailed GOM scans or borescope images, we can use the blade envelope to query whether a given blade needs to be refurbished or not.

The one high-level challenge that remains is how, in practice, the design, manufacturing and health monitoring teams cohesively converge and take advantage of a blade envelope, given that these teams are seldom collocated and may even be in different continents. To address this, we offer a simple plug-in from equadratures (used for doing the computational heavy lifting) \cite{seshadri2017effective} to a 3D modelling software package (we opt for Blender \cite{blender} given its open source nature). The latter can be easily adapted to industrial computer aided design (CAD) workflows.

We present a CAD representation of the controlled loss and mass flow rate blade envelope, shown in Figure~\ref{fig:cad_3}, in the Introduction. The purple and green airfoils correspond to profiles with negative and positive leading edge displacement respectively, just as plotted before, but now superimposed with the nominal blade (shown in black). \hl{Example invariant geometries can be highlighted for inspection, such as the one shown in blue here.} Our objective in showing these images is to demonstrate how these envelopes, once frozen for the objectives desired, can be 3D printed---either at scale or as a scaled-up model---and can sit on the desktops of designers, manufacturing engineers, and engine maintenance inspectors (Figure~\ref{fig:cad_4}). \hl{With these 3D visualizations showing displacements to scale, we gain insights to numerous queries related to the manufacturing process, a few of which are captured below.}
\begin{enumerate}
\item \hl{Guiding design trade-offs, such as the feasibility of increasing trailing edge thickness without loss of performance.}
\item \hl{Informing engineers where to focus scanning efforts via the control zone. }
\item \hl{Comparing the tolerance implications across multiple nominal designs with different corresponding blade envelopes.}
\end{enumerate}
These models can easily be transported, or indeed printed at different sites, and used to foster discussions on design and tolerance decisions. For completeness, close-up and isometric views of this blade envelope are shown in Figures~\ref{fig:cad_1} and \ref{fig:cad_2}. 

\begin{figure}
\centering
\includegraphics[width=0.99\linewidth]{figures/cad_4.png}
\caption{The blade envelope from Figure~\ref{fig:cad_3} can be suitably scaled for 3D printing and placed on desktops.}
\label{fig:cad_4}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=0.99\linewidth]{figures/cad_1_small.png}
\caption{An isometric view of the blade envelope in Figure~\ref{fig:cad_3}.}
\label{fig:cad_1}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.99\linewidth]{figures/cad_2_small.png}
\caption{Close-up of the leading edge of the blade envelope in Figure~\ref{fig:cad_3}. The demarcated iso-contour lines denote displacements at 5, 10 and 15 mm away from the nominal blade.}
\label{fig:cad_2}
\end{figure*}





==> intro.tex <==
\section{INTRODUCTION}

In the first part of this two-part paper \cite{wong_blade_nodate}, we defined the concept of a \emph{blade envelope}, leading to a computational guideline yielding automatic scrap-or-use decisions for manufactured turbomachinery components \hl{based on models trained from an aerodynamic database}. Using the theory of inactive subspaces, a range of geometric designs that are invariant in loss is identified, and geometries from this invariant region can be generated with no additional computational fluid dynamics (CFD) solves. \hl{From these geometries, we construct the blade envelope as the distribution of invariant geometries within a control zone. This enables us to calculate the distance of test profiles from the blade envelope using the statistical metric of Mahalanobis distance to gauge whether the profile is expected to give similar-to-nominal performance. Thus, the decision to scrap or keep a measured component reduces down to the computation of this distance from the blade envelope.} \hl{Throughout this two-part paper, we use the Von Karman Institute LS89 linear turbine cascade }{\cite{arts_aero-thermal_1992}} \hl{ with conditions as described in Section 2 of Part I for demonstration, but note that the base methodology of blade envelopes extends beyond 2D axial designs.}

In this second part, we extend blade envelopes beyond the manufacturing stage of production, and describe how they can be used during the design stage as well.  During the shape design of a highly-loaded turbine stage, the minimization of loss is often accompanied with constraints to avoid trivial solutions where the blade is unloaded. For example, in \cite{torreguitart_optimization_2018}, the exit flow angle is constrained to be above the baseline value to ensure sufficient work extraction. In \cite{montanelli_gradient_2015}, the authors put an equality constraint on the mass flow rate while optimizing the loss coefficient to factor out possible reduction in entropy generation due to reduction in flow capacity. Prior work \cite{seshadri_yuchi_parks_shahpar_2020, seshadri_turbomachinery_2017} has leveraged active subspaces to construct 2D performance maps for compressor blade design. In the latter work, multiple objectives including the pressure ratio and flow capacity are considered by mapping contours of different objectives onto the active subspace of efficiency. Manufacturing deviations are modeled as constant excursions from the nominal design. The main drawback of this approach is the requirement to run further simulations to map out performance contours in the active subspace. In this work, we incorporate multiple aerodynamic design requirements by interpreting them as additional constraints factored into blade envelopes. \hl{In upcoming future work, we extend our scope of consideration to structural requirements, and examine its implications on the tolerance covariance as additional constraints. }

In situations where tighter control over the performance of the component is required, constraints on surface flow characteristics can be implemented. Clark \cite{clark_step_2019} establishes the correlation between aerodynamic features---defined via parts of the surface isentropic Mach number distribution---and aerodynamic performance. Control over these key features can be achieved by factoring the isentropic Mach number distribution as an additional \emph{vector-valued} objective in blade envelopes. This approach is similar in spirit to \emph{inverse design}, where a target distribution is specified on the surface of a blade, and the blade shape is iteratively modified to give a geometry that matches the distribution. While inverse design yields an optimal geometry that fits the design criterion over the entire surface, our approach aims to find designs that satisfy the target distribution in \hl{locations} that are most critical to performance. The relaxation of constraints on other locations allows a range of designs to be specified, whose expanse is explicitly quantified by the blade envelope. Moreover, we can combine the control over the surface flow profile with constraints over other scalar objectives to perform inverse design constrained by requirements on other measures of performance.

In addition to computationally quantifying the region of a high-dimensional design space corresponding to designs with invariant objective values, blade envelopes are also amenable to intuitive visualizations. We conclude this work by connecting the numerical output of the blade envelopes workflow to 3D modelling software, producing outputs such as Figure~\ref{fig:cad_3}. The result is a visualization of the possible designs within the blade envelope that can be easily shared between engineers and made interactive via novel technologies such as 3D printing and augmented reality. 

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figures/cad_3_small.png}
\caption{A CAD representation of the controlled loss and mass flow rate blade envelope, \hl{highlighting one distinct invariant profile in blue.} \hl{Note: In all 2D and 3D plots in this paper, all deformations are drawn to scale.}}
\label{fig:cad_3}
\end{figure}

%In section \cref{sec:intersection}, we discuss computational algorithms to extend the capability of blade envelopes to handle multiple objectives. 

%In this paper we talk about:
%\begin{enumerate}
%\item Multiple objectives and their intersection and why the intersection notion is more powerful than prior work on mapping.
%\item Vector-valued dimension reduction -- contrasting average from intersection.
%\item Recipes for inverse design
%\item Testing again.
%\end{enumerate}


==> method.tex <==
\section{COMPUTATIONAL METHODOLOGIES}

Blade envelopes demarcate boundaries between regions within the space of manufactured geometries which exhibit similar performance metrics, \hl{one of which is shown in blue in Figure~{\ref{fig:cad_3}}}.  These envelopes are formed from statistics derived from an aerodynamic database containing geometries sampled from the inactive subspace with respect to a scalar objective. Building upon this framework, we describe two algorithms to identify regions of the design space characterized by invariance in \emph{multiple objectives}, including both scalar- and vector-valued objectives. This enables us to obtain samples invariant in these objectives to form the required database for a multi-objective blade envelope.

Recall from \cite{wong_blade_nodate} the partitioning of the design space into the \emph{active} and \emph{inactive} subspaces via an orthogonal matrix $\mQ = \left[\begin{array}{cc}
\mW & \mV \end{array}\right]$,
\begin{equation}
\vx = \mW \mW^{T} \vx + \mV \mV^{T} \vx,
\end{equation}
where we desire that the quantity of interest varies predominantly with changes in the active coordinates $\mW^T \vx$, and are approximately invariant with respect to changes in the inactive coordinates $\mV^T \vx$. Building on this idea of subspace decomposition, we aim to identify an inactive subspace matrix $\mV$ whose columns form a basis for a subspace within which multiple objectives are approximately invariant.

\subsection{Intersection of inactive subspaces} \label{sec:intersection}

% Consider two independent objectives $f_1(\vx)$ and $f_2(\vx)$ depending on the design variables $\vx$ differently. We can compute their respective gradient covariance matrices,
Consider two independent objectives $f_1(\vx)$ and $f_2(\vx)$ depending on the design variables $\vx$ differently. Assuming each objective is differentiable, we can compute the following symmetric positive semi-definite matrices,
\begin{equation}
\label{eqn:grad_cov}
\mC_i = \int_{\mathcal{X}} \nabla_{\vx} f_i(\vx) \nabla_{\vx} f_i(\vx)^T~ \tau~ d\vx, \qquad i=1,~2
\end{equation}
where $\tau = 2^{-d}$ defines a uniform distribution over the design space, which is a $d$-dimensional hypercube $[-1,1]^d$ as before. Their respective eigenvalue decompositions can be evaluated,
\begin{equation} \label{eqn:eig_decomp}
\mC_i = [\mW_i \enskip \mV_i] \begin{bmatrix}
\mLambda_{i,1} & \mathbf{0}\\
\mathbf{0} &\mLambda_{i,2}
\end{bmatrix}
\begin{bmatrix}
\mW_i^T\\
\mV_i^T
\end{bmatrix}, \qquad i=1,~2,
\end{equation}
where the non-negative eigenvalues are ordered in descending
order, and the diagonal terms in $\Lambda_{i,2}$ are sufficiently close to zero, for $i=1,2$.
From \cref{eqn:eig_decomp}, the inactive subspace corresponding to $f_i(\vx)$, i.e., the column span of $\mV_i$, can be obtained. Let's denote this by $\mathcal{V}_i = \text{colspan}(\mV_i)$. The idea is to find the  \emph{intersection} of the inactive subspaces $\mathcal{V}_{int} =  \mathcal{V}_1 \cap \mathcal{V}_2$. If a design perturbation lies within $\mathcal{V}_{int}$, then by definition it lies in both $\mathcal{V}_1$ and $\mathcal{V}_2$, implying that such a perturbation has insignificant effects on both $f_1(\vx)$ and $f_2(\vx)$. How do we find this intersection, and how can we sample from it?

It can be shown that $\mathcal{V}_{int}$ is a linear subspace that can be expressed as the column span of a basis matrix (see \cite[p.~64]{golub2013matrix}). Let this matrix be $\mV_{int}$. Once we can evaluate $\mV_{int}$, the exploration of the subspace $\mathcal{V}_{int}$ subject to constraints reduces to an application of the hit-and-run sampling algorithm as described in Part I \cite{wong_blade_nodate}. To find this matrix, we require the \emph{active} subspace basis matrices $\mW_1 \in \myRe^{d\times r_1}$ and $\mW_2 \in \myRe^{d\times r_2}$,
%and the assumption that the total number of dimensions of the active subspaces $r_1+r_2$  is less than $d$,
and the assumption that the dimension $r$ of the space $\text{colspan}(\mW_1) \oplus \text{colspan}(\mW_2)$ is less than $d$, the ambient design space dimension, where $\oplus$ denotes the direct sum. With these assumptions, the following recipe can be used to find $\mV_{int}$:
\begin{enumerate}
\item Form $\mW_{both} := [\mW_1 \enskip \mW_2]$.
\item Decompose $\mW_{both}$ by QR-factorization, $\mW_{both} = \mQ \mR$.
\item Set $\mV_{int}$ to be the last $d - r$ columns of $\mQ$.
\end{enumerate}
This gives us the basis matrix $\mV_{int}$ corresponding to the inactive subspace for both $f_1(\vx)$ and $f_2(\vx)$. This procedure is straightforwardly generalizable to $n>2$ objectives via induction, as long as the dimension $r$ of the direct sum of the active subspaces is strictly less than $d$.

\subsection{Vector-valued objectives} \label{sec:vecdr}

Given the method of intersections, a natural extension to find an invariant subspace for a vector-valued objective would be to treat the $N$ components of the objective
\begin{align} \label{eqn:discrete_M}
\begin{split}
\mathbf{M(x)} &= [M_1(\vx),~M_2(\vx),~...,~M_N(\vx)]\\
&= [M_1,~M_2,~...,~M_N]
\end{split}
\end{align}
as independent scalar objectives, and find the intersection of all their respective inactive subspaces $\mathcal{V}_{int} = \mathcal{V}_1 \cap \mathcal{V}_2 \cap ... \cap \mathcal{V}_N$. The challenge with this approach for large $N$ (when compared to $d$) is the fact that the total number of active coordinates is likely to exceed $d$. In this situation, the intersection of the inactive subspaces is trivial, i.e., it contains only the zero vector. An alternative approach that provides approximate invariance across the component objectives is required.

We take cues from the work of Wong et al. \cite{WONG2020113383} and Zahm et al. \cite{zahm_gradient-based_2018} and define the following multivariate generalisation of \eqref{eqn:grad_cov},
%a gradient covariance matrix for the vector valued objective,
\begin{equation}
\mH = \int_{\mathcal{X}} \mJ(\vx)~\mR~\mJ(\vx)^T~ \tau~ d\vx,
\end{equation}
where
\begin{equation}
\mJ \left( \vx \right) = \left[ \frac{\partial M_{1}}{\partial \vx} ,~ \ldots~ , \frac{\partial M_{N}}{\partial \vx} \right] \in \myRe^{d\times N}
\end{equation}
is the Jacobian matrix. The matrix $\mR$ is a user-defined $N\times N$ diagonal \emph{weight matrix},
\begin{equation}
\mR=\begin{bmatrix}
\omega_1 &&&\\
& \omega_2 &&\\
&& \ddots &\\
&&& \omega_N
\end{bmatrix},
\end{equation}
 where $\omega_i \geq 0$ for $1\leq i \leq N$. The corresponding active and inactive subspace basis matrices $\mW_M$ and $\mV_M$ for $\mathbf{M}$ can be found again via the eigenvalue decomposition,
\begin{equation}
\mH = [\mW_M \enskip \mV_M] \begin{bmatrix}
\mLambda_{M,1} & \mathbf{0}\\
\mathbf{0} &\mLambda_{M,2}
\end{bmatrix}
\begin{bmatrix}
\mW_M^T\\
\mV_M^T
\end{bmatrix},
\end{equation}
with $\mW_M \in \myRe^{d\times r}$ and $\mV_M \in \myRe^{d\times (d-r)}$. The dimensionality $r$ is found by identifying the largest eigenvalue gap, as in the scalar case. In \cite{zahm_gradient-based_2018}, the focus is placed on finding the active subspace for vector-valued objectives to achieve dimension reduction. Here, we place the emphasis on the inactive subspace instead, to achieve component-wise invariance in vector-valued quantities.

The power of this method lies in the flexibility in setting the weight matrix $\mR$. It can be shown that $\mH$ is the weighted sum of the gradient covariance matrices corresponding to each component objective \cite[Sec.~5.2.2]{zahm_gradient-based_2018}. That is, if
\begin{equation}
\mC_i = \int_{\mathcal{X}} \nabla_{\vx} M_i(\vx) \nabla_{\vx} M_i(\vx)^T~ \tau~ d\vx,
\end{equation}
then
\begin{equation}
\mH = \sum_{i=1}^N \omega_i \mC_i.
\label{equ:H}
\end{equation}
The larger the weight for $\omega_i$, the bigger its influence on the eigenvectors $\mW_M$ and $\mV_M$.  Samples from the inactive subspace yield output values that are close to nominal at locations with a large prescribed weight; in locations with a smaller weight, output values are allowed to vary more freely. The weights allow us to prescribe different degrees of invariance to various locations indexed by the vector-valued objective.

\subsection{Discussion: Distinguishing between inactive subspaces}

The problem of finding an orthonormal basis for the intersection of multiple inactive subspaces is equivalent to finding the null space of their direct sum (see 6.4.2 in \cite{golub2013matrix}). In other words, there is a connection between the inactive subspace of $\mH$ from \eqref{equ:H}, and last few columns of $\mQ$ in \Cref{sec:intersection}.

Consider the inactive subspace to be the orthogonal complement of the column span of $\mH$, which would correspond to the eigenvectors of $\mH$ that have eigenvalues of zero. In practice, however, if we have many independent objectives, there is a strong possibility that the span of $\mH$ will have full dimension, in which case the inactive subspace will be trivial, i.e., $\left\{ \boldsymbol{0} \right\}$. For practical reasons, this motivates us to consider a relaxed definition of the inactive subspace, which corresponds to the linear span of \emph{small} eigenvalues of $\mH$. The threshold between \emph{small} and \emph{not-small} is problem specific, although one can make various scaling arguments about what a reasonable threshold would be. In this setting, the inactive subspace will depend strongly on the choice of the scaling parameters $\mR$, which can weight the relative importance of difference subspaces.

Utilizing the direct intersection approach in \Cref{sec:intersection} implies that the inactive subspaces of the various objectives are characterized by eigenvalues that are all exactly zero (albeit with a different formulation of the active subspace). We can interpret this as a \emph{strongly} inactive subspace, and it will be used when considering multiple flow quantities. In contrast, the inactive subspace obtained through $\mH$ represents a \emph{weakly} inactive subspace, and is used in this paper for studying a single vector-valued quantity, e.g., isentropic Mach number distribution.

%\subsection{Discussion: Intersection or Average?}
%\todo[inline]{Isn't this comparing apples with oranges? The idea in \cite{zahm_gradient-based_2018} is about finding the active subspace, and not the inactive subpsace.  The orthogonal complement of their output will give you the inactive subspace.}
%\textcolor{green}{It should be clear that the intersection of subspaces and taking the orthogonal complement of the active subspace generated from an average of gradient covariance matrices (the averaging method) are two mathematically different operations. Although the vector-valued ideas in \cite{zahm_gradient-based_2018} focus on the averaging approach, we argue that the intersection may be more appropriate under certain circumstances.}

%When the number of objectives is small compared with the number of input dimensions---with no inherent notion of relative importance---the intersection method provides a non-trivial inactive subspace. Samples obtained using this method usually yield output quantities of interest closer to their nominal values than samples obtained by treating the objectives as a vector-valued objective.

%On the other hand, if the number of objectives is comparable to $d$, it is more advisable to use the averaging method, because the intersection of all the inactive subspaces is likely to be trivial. A suitable weighting should be enforced in the computation of the gradient covariance matrix of the vector-valued objective, preferably localizing the invariance to some subset of the components. This increases the likelihood that a clear eigenvalue gap exists.

%To summarize, the averaging method should be used for inherently vector-valued objectives, such as a flow quantity defined over the surface of a component, where the number of components is larger than the number of design variables. For a small number of distinct objectives, the intersection of their inactive subspaces provides tighter control over the variance in each objective. The two approaches should be combined when different types of objectives need to be accounted for.

\subsection{Constrained tuning via active coordinates} \label{sec:inverse_design_method}

Assuming that the active subspaces are linearly independent---a mild assumption for independent objectives, using the method of intersection of $n$ scalar- or vector-valued objectives, we obtain a linear decomposition of the design space. This decomposition can be characterised by gathering the active subspace basis matrices together with the intersection of the inactive subspaces,
\begin{equation}
\mD = \begin{bmatrix}
\mW_1 & \mW_2 & ... & \mW_n & \mV
\end{bmatrix},
\end{equation}
yielding a square matrix $\mD \in \myRe^{d\times d}$ with independent columns. Corresponding to $\mD$, a coordinate transformation on the design $\vx$ yields the following
\begin{align}
\begin{split}
\mD^T \vx &= \begin{bmatrix}
\left(\mW_1^T \vx\right)^T & \left(\mW_2^T \vx\right)^T & ... & \left(\mW_n^T \vx\right)^T & \left(\mV^T \vx\right)^T
\end{bmatrix}^T\\
&= \begin{bmatrix}
\smash[b]{\block{r_1+r_2+...+r_n}} & \vz^T\\
\end{bmatrix}^T
\end{split}
\end{align}
The first components of the new coordinates $\vu_1, \vu_2,...,\vu_n$ correspond to the active coordinates of the objectives $f_1, f_2,...,f_n$; the final coordinates $\vz$ correspond to the inactive coordinates. Any perturbation lying in the column space of $\mV$ has its first $r_1+r_2+...+r_n$ coordinates equal to zero, implying that it causes no change to the active coordinates for all objectives. Thus, this perturbation does not cause significant change to any objective.

Assuming that each coordinate is independent, the active coordinates can also be treated as tunable parameters that directly control each objective separately. Adjusting the values of $\vu_1$ while keeping every other active coordinate constant results in changes in $f_1$, while maintaining the values of other objectives. Note that we can allow the inactive coordinates $\vz$ to float, since those coordinates do not affect any objective.


==> pauls-macros.tex <==
% Lots of macros. Thanks to D.F. Gleich for a bunch of these. 
\usepackage{bm}

%%\graphicspath{{./}{./figs/}}

  \def\clap#1{\hbox to 0pt{\hss#1\hss}}
  \def\mathclap{\mathpalette\mathclapinternal}
  \def\mathclapinternal#1#2{%
    \clap{$\mathsurround=0pt#1{#2}$}}

\providecommand{\mat}[1]{\bm{#1}}%
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\vecalt}[1]{\bm{#1}}

% Commands
% bold upper case
\providecommand{\eye}{\mat{I}}
\providecommand{\mA}{\ensuremath{\mat{A}}}
\providecommand{\mB}{\ensuremath{\mat{B}}}
\providecommand{\mC}{\ensuremath{\mat{C}}}
\providecommand{\mD}{\ensuremath{\mat{D}}}
\providecommand{\mE}{\ensuremath{\mat{E}}}
\providecommand{\mF}{\ensuremath{\mat{F}}}
\providecommand{\mG}{\ensuremath{\mat{G}}}
\providecommand{\mH}{\ensuremath{\mat{H}}}
\providecommand{\mI}{\ensuremath{\mat{I}}}
\providecommand{\mJ}{\ensuremath{\mat{J}}}
\providecommand{\mK}{\ensuremath{\mat{K}}}
\providecommand{\mL}{\ensuremath{\mat{L}}}
\providecommand{\mM}{\ensuremath{\mat{M}}}
\providecommand{\mN}{\ensuremath{\mat{N}}}
\providecommand{\mO}{\ensuremath{\mat{O}}}
\providecommand{\mP}{\ensuremath{\mat{P}}}
\providecommand{\mQ}{\ensuremath{\mat{Q}}}
\providecommand{\mR}{\ensuremath{\mat{R}}}
\providecommand{\mS}{\ensuremath{\mat{S}}}
\providecommand{\mT}{\ensuremath{\mat{T}}}
\providecommand{\mU}{\ensuremath{\mat{U}}}
\providecommand{\mV}{\ensuremath{\mat{V}}}
\providecommand{\mW}{\ensuremath{\mat{W}}}
\providecommand{\mX}{\ensuremath{\mat{X}}}
\providecommand{\mY}{\ensuremath{\mat{Y}}}
\providecommand{\mZ}{\ensuremath{\mat{Z}}}
\providecommand{\mLambda}{\ensuremath{\mat{\Lambda}}}
\providecommand{\mSigma}{\ensuremath{\mat{\Sigma}}}
\providecommand{\mzero}{\ensuremath{\mat{0}}}

\providecommand{\ones}{\vec{e}}
\providecommand{\va}{\ensuremath{\vec{a}}}
\providecommand{\vb}{\ensuremath{\vec{b}}}
\providecommand{\vc}{\ensuremath{\vec{c}}}
\providecommand{\vd}{\ensuremath{\vec{d}}}
\providecommand{\ve}{\ensuremath{\vec{e}}}
\providecommand{\vf}{\ensuremath{\vec{f}}}
\providecommand{\vg}{\ensuremath{\vec{g}}}
\providecommand{\vh}{\ensuremath{\vec{h}}}
\providecommand{\vi}{\ensuremath{\vec{i}}}
\providecommand{\vj}{\ensuremath{\vec{j}}}
\providecommand{\vk}{\ensuremath{\vec{k}}}
\providecommand{\vl}{\ensuremath{\vec{l}}}
\providecommand{\vm}{\ensuremath{\vec{l}}}
\providecommand{\vn}{\ensuremath{\vec{n}}}
\providecommand{\vo}{\ensuremath{\vec{o}}}
\providecommand{\vp}{\ensuremath{\vec{p}}}
\providecommand{\vq}{\ensuremath{\vec{q}}}
\providecommand{\vr}{\ensuremath{\vec{r}}}
\providecommand{\vs}{\ensuremath{\vec{s}}}
\providecommand{\vt}{\ensuremath{\vec{t}}}
\providecommand{\vu}{\ensuremath{\vec{u}}}
\providecommand{\vv}{\ensuremath{\vec{v}}}
\providecommand{\vw}{\ensuremath{\vec{w}}}
\providecommand{\vx}{\ensuremath{\vec{x}}}
\providecommand{\vy}{\ensuremath{\vec{y}}}
\providecommand{\vz}{\ensuremath{\vec{z}}}
\providecommand{\vpi}{\ensuremath{\vecalt{\pi}}}

% script upper case
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sE}{\mathcal{E}}
\newcommand{\sI}{\mathcal{I}}
\newcommand{\sJ}{\mathcal{J}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}

% script lower case
\newcommand{\sx}{\chi}

% bold greek
\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}

% some useful commands
\newcommand{\ip}[2]{\left\langle #1,\,#2\right\rangle}
\newcommand{\Exp}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Cov}[2]{\operatorname{Cov}\left[#1,\,#2\right]}
\newcommand{\Corr}[2]{\operatorname{Corr}\left[#1,\,#2\right]}
\newcommand{\Var}[1]{\operatorname{Var}\left[#1\right]}
\newcommand{\Prob}[2]{\mathbb{P}\left[#2\right]}
\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\ddx}[2]{\frac{\partial #1}{\partial x_{#2}}}
\newcommand{\argmax}[1]{\underset{#1}{\mathrm{argmax}}}
\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}}}
\newcommand{\mini}[1]{\stackrel{#1}{\mathrm{minimum}}}
\newcommand{\maxi}[1]{\stackrel{#1}{\mathrm{maximum}}}
%%\newcommand{\st}{\text{subject to}}
\newcommand{\trace}[1]{\operatorname{trace}\left(#1\right)}

